Frobenius templates in certain $2 \times 2$ matrix rings

The classical Frobenius problem is to find the largest integer that cannot be written as a linear combination of a given set of positive, coprime integers using nonnegative integer coefficients. Prior work has generalized the classical Frobenius problem from integers to Frobenius problems in other rings. This paper explores Frobenius problems in various rings of (upper) triangular $2 \times 2$ matrices with constant diagonal.

==> macro.tex <==
\newcommand{\nat}{\mathbb{N}}
\newcommand{\zz}{\mathbb{Z}}

\newcommand{\stin}{\subseteq}
\newcommand{\sstin}{\subset}
\newcommand{\gpin}{\leqslant}

\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\I}[1]{\mathscr{I}_{#1}}

\newcommand{\ques}{\noindent\textbf{Question:} }

\newcommand{\seqn}[1]{(#1)_{n=1}^\infty}
\newcommand{\seqk}[1]{(#1)_{k=1}^\infty}
\newcommand{\seqm}[1]{(#1)_{m=1}^\infty}
\newcommand{\gen}[1]{\left\langle#1\right\rangle}


\newcommand{\aut}{\textnormal{Aut}}
\newcommand{\mrd}{\textnormal{mrd}}
\newcommand{\en}{\textnormal{End}}
\newcommand{\pow}{\mathcal{P}}
\newcommand{\sym}{\textnormal{Sym}}

\newcommand{\sett}[1]{\left\{ #1 \right\}}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\paren}[1]{\left( #1 \right) }
\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\ti}[1]{\textit{#1}}
\newcommand{\gspan}[2]{\langle #1 \rangle_{#2} }

\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\frob}[1]{\textnormal{Frob}\left( #1 \right)}
\newcommand{\frobt}[1]{\textnormal{Frob}_{\mb{T}}\left( #1 \right)}
\newcommand{\cond}[1]{\chi\left(#1 \right)}

